Pose-Guided Self-Training with Two-Stage Clustering for Unsupervised Landmark Discovery

Unsupervised landmarks discovery (ULD) for an object category is a challenging computer vision problem. In pursuit of developing a robust ULD framework, we explore the potential of a recent paradigm of self-supervised learning algorithms, known as diffusion models. Some recent works have shown that these models implicitly contain important correspondence cues. Towards harnessing the potential of diffusion models for the ULD task, we make the following core contributions. First, we propose a ZeroShot ULD baseline based on simple clustering of random pixel locations with nearest neighbour matching. It delivers better results than existing ULD methods. Second, motivated by the ZeroShot performance, we develop a ULD algorithm based on diffusion features using self-training and clustering which also outperforms prior methods by notable margins. Third, we introduce a new proxy task based on generating latent pose codes and also propose a two-stage clustering mechanism to facilitate effective pseudo-labeling, resulting in a significant performance improvement. Overall, our approach consistently outperforms state-of-the-art methods on four challenging benchmarks AFLW, MAFL, CatHeads and LS3D by significant margins.

==> sec/1_intro.tex <==


\section{Introduction}
\label{sec:intro}


% \noindent\textbf{Background:} %Detecting object landmarks is an important computer vision task. 
% Landmarks depict the shape and spatial configuration of an object in 3D space, particularly for non-rigid objects e.g., human and animal faces \cite{jakab2018unsupervised,sanchez2019object,mallis2023keypoints,khan2020animalweb}. As such, landmarks identify the location of specific object parts bearing particular semantic meaning and so conform to a configuration that is usually manually designed \cite{mallis2023keypoints}. 

\noindent\textbf{Background:} A large body of works approach landmark detection for an object category in a fully-supervised setting  \cite{bulat2017far,khan2017synergy,wang2019adaptive,miao2018direct,dong2018style,kumar2020luvli}, which assumes the availability of sufficiently annotated data by humans. Typical object categories for landmark detection include human faces or bodies. In these object categories, a significant number (around thousands) of annotated images are available \cite{sanchez2019object}. However, akin to other computer vision problems, acquiring a large collection of annotated images for detecting landmarks in an arbitrary object category might be very costly \cite{mallis2023keypoints}. Therefore, in this paper, we aim to discover object landmarks in an unsupervised manner.

\noindent\textbf{Challenges:} Unsupervised learning of object landmarks is a challenging problem mainly because of the following reasons. Although landmarks are indexed with spatial coordinates, they convey high-level semantic information about object parts which is inherently difficult to learn without human supervision \cite{sanchez2019object, awan2023unsupervised}. %The variability in landmark configurations even for object categories like human faces render them ambiguous innately \cite{mallis2020unsupervised}. 
Detected landmarks should be invariant to different viewpoints, occlusions, and other appearance variations and also capture the shape perception of non-rigid objects, such as human faces \cite{sanchez2019object, mallis2023keypoints}. 
Some existing approaches to unsupervised landmark detection focus on learning strong representations, that can be mapped to manually annotated landmarks utilizing a few labeled images \cite{thewlis2017unsupervised_dense} or leverage proxy tasks, such as imposing equivariance constraints \cite{thewlis2017unsupervised, thewlis2017unsupervised_dense,thewlis2019unsupervised} or appending conditional image generation \cite{jakab2018unsupervised, sanchez2019object, zhang2018unsupervised, awan2023unsupervised}. %Approaches based on equivariance constraint requires that the landmark detector's output should be invariant to certain synthetic image deformation and this is treated as an optimization objective. 
%Methods leveraging image reconstruction as a proxy task require the reconstruction of a deformed image through a generator network that is conditioned on the output of the landmark detector. Often, the proxy task used is not tightly related to the actual task of landmark detection \cite{jakab2018unsupervised, sanchez2019object}. Consequently, 
Although obtaining promising performance, these methods struggle under different intra-class variations of object, such as large changes in pose and expression (see Fig.~\ref{fig:teaser}).

\noindent\textbf{Motivation:} Towards handling these challenges in unsupervised landmark discovery, in this paper, we explore the potential of a popular category of self-supervised learning models known as diffusion-based generative models \cite{ho2020denoising, song2020score}. Some recent works have shown the utility of diffusion models beyond image synthesis, for instance, these models can produce plausible results for other tasks, such as image editing \cite{meng2021sdedit, brooks2023instructpix2pix} and image-to-image translation \cite{parmar2023zero}. As such, these models are capable of converting one object into another object without modifying the pose and context of the former \cite{tang2023emergent}. This suggests the presence of implicit correspondence cues in the internal representations of diffusion models for different object classes \cite{luo2023diffusion,tang2023emergent, zhang2023tale}. %Such correspondence information 

\noindent\textbf{Contributions:} 
\begin{itemize}%[topsep=-3pt, noitemsep]
    \item To explore diffusion models for unsupervised landmark detection, we begin with a simple clustering of their pretrained internal representations indexed at randomly sampled pixel locations from object RoIs. For inference, we use nearest neighbour querying of randomly sampled pixel locations from unseen object image for discovering landmarks. Surprisingly, this \emph{zero-shot baseline} surpasses the existing best methods.
%a  simple clustering of the zero-shot internal representations of the diffusion model, corresponding to randomly sampled pixel locations from object RoIs, followed by nearest neighbour querying of randomly sampled pixel locations of an unseen object image for discovering landmarks. 
 \item Motivated by ZeroShot baseline, we develop an \emph{unsupervised landmark detection algorithm built on diffusion features}, namely D-ULD, that uses clustering for pseudo-labelling which are then used for self-training. %to learn correspondences across object images. 
We note that, this simple algorithm produces superlative results and bypasses competing methods by visible margins. 

\item We capitalize on D-ULD and introduce \emph{a new pose-guided proxy task} which reconstructs landmark heatmaps after producing  latent pose codes. 
Finally, to better capture the variations (e.g., caused by 3D rotations) in landmark representations in clustering process, we leverage these latent pose codes to develop \emph{a two-stage clustering mechanism} for better pseudo-labels, resulting in further performance improvement. The inclusion of pose-guided proxy task and two-stage clustering in D-ULD results in a robust unsupervised landmarks detection algorithm D-ULD++ (see Fig.~\ref{fig:teaser}). 

\item Extensive experiments on four challenging datasets, featuring human faces and cat faces, reveal that D-ULD++ consistently achieves remarkable performance across all datasets. 
\end{itemize}
%Moreover, an important feature of our method is the \emph{unsupervised generation of latent pose code} which can be exploited in various ways to induce auxiliary information into the unsupervised landmark detection pipeline.  

\begin{figure*}[!th]
    \centering
    \includegraphics[width=0.70\textwidth]{./figs/duldpp_architecture_diagram.pdf}
    \caption{
    %The network architecture consists of a frozen Stable Diffusion module, an aggregator network $\Psi_b$, a descriptor  $\Psi_f$ and detector head $\Psi_d$.$\Psi_d$ outputs a keypoint heat-map.    
     Proposed diffusion based unsupervised landmark detection algorithm: (a) D-ULD++ system diagram. (b) Pose-guided proxy task to improve self-training. (c) Two stage clustering to improve pseudo-labels. (d) Self-training using pseudo-labels.}
     % For D-ULD, during training we alternate between computing keypoint correspondences via clustering and self-training using these  correspondences. With D-ULD++ we introduce a pseudo-pose learning proxy task to encode the keypoint spatial configuration into latent codes via a variational auto-encoder (VAE). We then perform a two-stage clustering. We cluster the latent codes into pseudo-pose clusters. Then for the images corresponding to the latent codes within each cluster, we further cluster the keypoints giving more fine-grained, pose specific keypoints which we use for self-training the network.}
    \label{fig:architecture_diagram}
\end{figure*}

\section{Related Work}
\label{sec:related_work}

\noindent\textbf{Unsupervised Landmark Detection (ULD):} An early attempt towards ULD involved enforcing equivariant constraint on a landmark detector. This constraint provides  self-supervision by requiring the features produced by a detector to be invariant to the geometric transformations of an image. For ULD, equivariant constraints on image and pre-defined deformations were used along with auxiliary losses, such as locality \cite{thewlis2019unsupervised, thewlis2017unsupervised_dense}, diversity \cite{thewlis2017unsupervised} and others \cite{cheng2021equivariant}.  Albeit effective in discovering landmarks, as such approaches relying on equivariance constraint could struggle to produce semantically meaningful landmarks, especially under large intra-class variations \cite{mallis2023keypoints}.

A promising class of methods proposed conditional image generation as a proxy task where the landmark detector is required to produce the geometry of an object \cite{jakab2018unsupervised, sanchez2019object, awan2023unsupervised}. 
%In this pipeline, a landmark detector is tasked to capture the geometry of an object, which is then used along with a deformed image by a decoder to reconstruct the original image. 
The two distinct components in this pipeline are: a geometry distilled bottleneck and a conditional image generator. % \cite{jakab2018unsupervised, sanchez2019object}. %The detector and bottleneck are responsible for producing object's geometry which is then combined with the deformed version of an input image and sent to a conditional image generator for reconstructing the original version of the input image. 
Zhang et al. \cite{zhang2018unsupervised} considered landmark discovery as an intermediate step of image representation learning and proposed  to predict landmark coordinates  utilizing soft constraints. Others integrated image generation and equivariance constraints to obtain landmark representations \cite{cheng2021equivariant, kulkarni2019unsupervised, lorenz2019unsupervised}.
 %\cite{kulkarni2019unsupervised} introduced a keypoint bottleneck to transport learned image features between video frames; obtaining keypoints that consistently track objects and their parts.
%
Lorenz et al. \cite{lorenz2019unsupervised} disentangled shape and appearance  leveraging equivariance and invariance constraints. Wiles et al. \cite{wiles2018self} proposed a self-supervised learning for facial attributes from unlabeled videos which are then utilized to predict landmarks by training a linear layer on top of learned embedding. Most of these methods are prone to detecting semantically irrelevant landmarks under large pose variations.




\noindent\textbf{Clustering driven Self-Training:} In self-training methods, a model's own predictions are utilized as pseudo-labels (PLs) for generating training signal. Typical approaches utilize highly confident predictions as hard PLs \cite{sohn2020fixmatch, xie2020self}, or via model ensembling \cite{nguyen2019self}. Self-training has been mostly leveraged for image classification task \cite{sohn2020fixmatch, xie2020self, rizve2020defense}, however, some works focus on unsupervised semantic segmentation \cite{dai2015boxsup, khoreva2017simple} and salient object detection \cite{zhang2017supervision}.
%
Some other self-training methods use clustering to construct pseudo-labels \cite{asano2019self, caron2018deep, caron2020unsupervised, noroozi2018boosting, yan2020clusterfit, zhuang2019local}. Typically, the clustering serves to assign PLs for the unlabelled training images. The PLs are then used to create supervision \cite{caron2018deep, noroozi2016unsupervised}. Some other related methods are slot-attention mechanisms \cite{kipf2021conditional, locatello2020object}. 
A few mapped image patches into a categorical latent distribution of learnable embeddings \cite{razavi2019generating, van2017neural}, and proposed routing mechanisms based on soft-clustering \cite{lee2019set}. %The primary goal in these methods is to learn a powerful feature representation in an unsupervised way that can be applied to downstream tasks \cite{mallis2023keypoints}. 
In unsupervised landmark discovery, the work of Mallis et al. \cite{mallis2020unsupervised, mallis2023keypoints} forms landmark correspondence through clustering landmark representations. This clustering is used to select pseudo-labels for first stage self-training. We also cluster landmark representations to generate PLs, however, we use it to propose a landmark detection method based on stable diffusion.% model.

\noindent\textbf{Diffusion Model:} Diffusion models \cite{song2019generative, song2020score,ho2020denoising} belong to the potent family of generative models. The Ablated Diffusion \cite{dhariwal2021diffusion} showcased that diffusion models can generate better quality images on ImageNet \cite{deng2009imagenet} compared to GANs. Later, classifier-free guidance \cite{ho2022classifier} and latent diffusion model \cite{rombach2022high} facilitated its scaling to large collection of image-text pairs \cite{schuhmann2022laion}, thereby democratising high-resolution image synthesis. This lead to the introduction of popular open-sourced text-to-image diffusion model, namely Stable Diffusion. Owing to its superlative generation capability, some works began exploring the internal representations of diffusion models \cite{tumanyan2023plug, hertz2022prompt, baranchuk2021label, xu2023open}. For instance, \cite{baranchuk2021label, xu2023open} investigate adapting pre-trained diffusion model for downstream recognition tasks. Different to these methods, we explore the potential of pre-trained Stable Diffusion for ULD.

% for first and second stages in the method. The pseudo-labels are then used to learn a landmark detector in a supervised manner in the second stage.

%by thresholding highly confident predictions and retaining confident predictions . 



==> sec/2_formatting.tex <==
\section{Related Work}
\label{sec:related_work}

\noindent\textbf{Unsupervised Landmark Detection:} An early attempt towards unsupervised landmark detection involved enforcing equivariant constraint on a landmark detector. As such, this constraint provides a self-supervisory signal by requiring the features produced by a detector to be invariant to the geometric transformations of an image. For discovery landmarks, equivariant constraints on image and pre-defined deformations were used along with auxiliary losses, such as locality \cite{thewlis2019unsupervised, thewlis2017unsupervised_dense} and diversity \cite{thewlis2017unsupervised}, to avoid trivial solutions for the landmark detector. Albeit effective in discovering landmarks, as such approaches relying on equivariance constraint could struggle to produce semantically meaningful landmarks \cite{mallis2023keypoints}.

An alternate and promising direction proposed conditional image generation as a proxy task where the landmark detector is required to produce geometry of an object. 
%In this pipeline, a landmark detector is tasked to capture the geometry of an object, which is then used along with a deformed image by a decoder to reconstruct the original image. 
The two distinct components in this pipeline are: a geometry distilled bottleneck and a conditional image generator \cite{jakab2018unsupervised, sanchez2019object}. The detector and bottleneck are responsible for producing object's geometry which is then combined with the deformed version of an input image and sent to a conditional image generator for reconstructing the original version of the input image. The work of \cite{zhang2018unsupervised} considers landmark discovery as an intermediate step of image representation learning and proposed a neural network to predict landmark coordinates and utilizes soft constraints to validate detected landmarks. 
With similar motivation, some methods integrate image generation and equivariance constraint to obtain object feature representation \cite{cheng2021equivariant, kulkarni2019unsupervised, lorenz2019unsupervised}
Likewise, \cite{cheng2021equivariant} 
showed that, effective object feature representation for predicting landmarks emerge after imposing equivariance constraints. 
\cite{kulkarni2019unsupervised} introduced a keypoint bottleneck to transport learnt image features between video frames; obtaining keypoints that consistently track objects and their parts.
%
The work of \cite{lorenz2019unsupervised} proposed to disentangle shape and appearance and leveraged equivariance and invariance constraints into the generative framework. Wiles et al. \cite{wiles2018self} proposed a self-supervised learning framework to learn facial attributes from unlabeled videos which are then utilized to predict landmarks by training a linear layer on top of learned embedding. Most of these methods are prone to detecting semantically irrelevant landmarks under large pose variations.

\noindent\textbf{Clustering driven Self-Training:} In self-training methods, a model's own predictions are utilized as pseudo-labels (PLs) for generating training signal. Typical approaches utilize highly confident predictions as hard PLs \cite{sohn2020fixmatch, xie2020self}, or via model ensembling \cite{nguyen2019self}. Self-training has been mostly leveraged for image classification task \cite{sohn2020fixmatch, xie2020self, rizve2020defense}, however, some works focus on unsupervised semantic segmentation \cite{dai2015boxsup, khoreva2017simple} and salient object detection \cite{zhang2017supervision}.

Another class self-training method use clustering to construct pseudo-labels \cite{asano2019self, caron2018deep, caron2020unsupervised, noroozi2018boosting, yan2020clusterfit, zhuang2019local}. Typically, the clustering serves to assign PLs for the unlabelled training images. The PLs are then used to create supervision via objectives such as Cross Entropy \cite{caron2018deep, noroozi2016unsupervised}. Some other related methods are slot-attention mechanisms \cite{kipf2021conditional, locatello2020object}, map image patches into a categorical latent distribution of learnable embeddings \cite{razavi2019generating, van2017neural}, and routing mechanisms based on soft-clustering \cite{lee2019set}. The primary goal in these methods is to learn a powerful feature representation in an unsupervised way that can be applied to downstream tasks. In unsupervised landmark discovery, the work of \cite{mallis2020unsupervised, mallis2023keypoints} forms landmark correspondence through clustering landmark representations. This clustering is used to select pseudo-labels for first stage self-training. We also cluster landmark representations to generate PLs, however, we use it to propose a landmark detection pipeline based on stable diffusion model.

\noindent\textbf{Diffusion Model:} The class of diffusion model \cite{song2019generative, song2020score,ho2020denoising} belongs to the potent family of generative models. The Ablated Diffusion work \cite{dhariwal2021diffusion} showcased that, compared to generative adversarial networks (GANs), diffusion model can generate better quality images on ImageNet \cite{deng2009imagenet}. Later, classifier-free guidance \cite{ho2022classifier} and latent diffusion model \cite{rombach2022high} facilitated its scaling to large collection of image-text pairs \cite{schuhmann2022laion}, thereby democratising high-resolution image synthesis. This lead to the introduction of popular open-sourced text-to-image diffusion model, namely Stable Diffusion. Owing to its superlative generation capability, some works began  exploring the internal representations of diffusion models \cite{tumanyan2023plug, hertz2022prompt, baranchuk2021label, xu2023open}. For instance, \cite{baranchuk2021label, xu2023open} investigate adapting pre-trained diffusion model for downstream visual recognition tasks. Different to aforementioned methods, we explore the potential of pre-trained Stable Diffusion for unsupervised object landmark discovery.

% for first and second stages in the method. The pseudo-labels are then used to learn a landmark detector in a supervised manner in the second stage.

%by thresholding highly confident predictions and retaining confident predictions . 

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/evaluation.tex <==
% \section{Experiments}
% \label{sec:experiments}

% %---------------------------------------------------------------------------------------
% %\subsection{Evaluation Metrics} % This will be changed, The original text will be written and replaced
% %\noindent\textbf{Evaluation metrics \& baselines:}
% \noindent\textbf{Datasets, Evaluation metrics \& Baselines:} We perform experiments on four diverse datasets: AFLW~\cite{koestinger2011annotated}, LS3D~\cite{bulat2017far}, CatHeads~\cite{zhang2008cat} and MAFL~\cite{liu2015deep}. We follow the same dataset splits and  evaluation protocol used in~\cite{mallis2023keypoints}. See supplementary material for details on datasets. 
% For evaluation, we use the standard metrics of \textbf{Forward} and \textbf{Backward} Normalized Mean-squared Error (\textbf{NME}) widely used for landmark detection \cite{sanchez2019object, mallis2020unsupervised, mallis2023keypoints}. %This metric involves training a simple regressor, which maps the detected landmarks to ground-truth landmarks. 
% In \textbf{Forward NME}, we train a regressor to map the discovered landmarks to the ground truth landmarks and compute NME\%. In the \textbf{Backward NME}, we train a regressor to map the ground truth landmarks to discovered landmarks and compute NME\%. %These two metrics collectively provide a comprehensive assessment of the accuracy and stability of our landmark detection method. 
% The mappings are learned using a random subset of images from the dataset. We use the same subset as~\cite{mallis2023keypoints}. 
% %\noindent\textbf{Baselines:} 
% We benchmark against the following baselines: Lorenz et al. ~\cite{lorenz2019unsupervised}, Shu et al.~\cite{sanchez2017functional}, Jakab et al.~\cite{jakab2018unsupervised}, Zhang et al.~\cite{zhang2018unsupervised}, Sanchez et al.~\cite{sanchez2019object}, Mallis et al.~\cite{mallis2023keypoints} and Awan et al.~\cite{awan2023unsupervised}. Additionally, as all these methods do not make use of diffusion models, so we also retrain Mallis with Stable Diffusion features via the same aggregator network that we use instead of its FAN~\cite{bulat2017far} backbone. We refer to this method as Mallis (D). We use $K=10$ and $M=100$ as in the original method using the same training protocol~\cite{mallis2023keypoints} .

% \noindent\textbf{Training details:} Training consists of 4 stages. \textbf{Bootstrapping: }The network $\Psi$ is intially trained with the with Adam~\cite{kingma2014adam} optimizer with learning
% rate $1\times 10^{-4}$
% and betas $(0.9, 0.999)$; trained for $50K$ iterations, with a batch size of 12 per GPU. \textbf{D-ULD:} After bootstrapping, we alternate between clustering and training the network using pseudo-ground truth every $5000$ iterations. We train for a total of $100k$ iterations for all four datasets. The margin $m$ used in the contrastive loss $\SL_f$ is set to $0.8$. We multiply $\SL_d$ with $0.2$ before training. \textbf{Pose Proxy-Task Training:} For this stage, we initialize the model $\Psi$ with the training of D-ULD, append the VAE $\Psi_V$ to the descriptor head $\Psi_d$. . For this stage, $\Psi_f$ is frozen and $\Psi_V$ is minimized by the ELBO loss. We reduce the learning rate for the Adam optimizer to $5 \times 10^{-5}$ and train for $50k$ iterations. \textbf{D-ULD++:} We discard the decoder of $\Psi_V$ and initialize the rest of the network weights with those obtained after proxy-task training. We train this network for $100k$ iterations using the Adam optimizer with the same parameters as before, but with a learning rate of $5\times 10^{-4}$. Every $5000$ iterations, we perform clustering and update the pseudo-ground truth.


% \begin{table*}[h]
% \small
%     \centering
%     \begin{tabular}{ccccccccc}
%     \textbf{Method} & \multicolumn{2}{c}{\textbf{MAFL}} & \multicolumn{2}{c}{\textbf{AFLW}} & \multicolumn{2}{c}{\textbf{LS3D}} & \multicolumn{2}{c}{\textbf{CatHeads}}\\
%           & F & B & F & B & F & B & F & B\\
%                   \hline
%       %Lorenz~\cite{lorenz2019unsupervised} (K=10) &  3.24 & \textbf{O} & \textbf{A} &  \textbf{B} & \textbf{C} & \textbf{D} &  9.30 & \textbf{F} \\
%       %Shu~\cite{sanchez2017functional} & 5.45 & \textbf{O} &  \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} & \textbf{E} & \textbf{F}\\
%       Jakab~\cite{jakab2018unsupervised} (K=10) &  \underline{3.19} & 4.53 & 6.86 & 8.84 & 5.38 & 7.06 & 4.53 & 4.06 \\
%       Zhang~\cite{zhang2018unsupervised} (K=10) & 3.46 & 4.91 & 7.01 & 8.14 & 6.74 & 7.21 & 4.62 &  4.15\\
%       Sanchez~\cite{sanchez2019object} (K=10) & 3.99 & 14.74 &  6.69 & 25.84  & 26.41 & 5.44 & 4.42 & 4.17\\
% %      Sahasrabudhe~\cite{sahasrabudhe2019lifting} & 6.01 & \textbf{O} & \textbf{E} & \textbf{F} & \textbf{A} & \textbf{B} & \textbf{C} & \textbf{D} \\
%       Mallis~\cite{mallis2023keypoints} &  \underline{3.19}   & \underline{4.23} & 7.37 & 8.89 &  6.53 & 6.57 &  9.31 & 10.08 \\
%       Awan~\cite{mallis2023keypoints} &  3.50   & 5.18 & \underline{5.91} &  \underline{7.96} & \underline{5.21} & \underline{4.69} & \underline{3.76} & \underline{3.94} \\
%       \hline
%       Mallis (D) & 2.74 & 3.11 &  3.38 & 3.75 & 2.89 &  3.76 & 3.14 & 3.62\\
%          Zero Shot (K=10) & 3.14 & 3.27 &  4.98 & 6.29 & 3.53 &  4.14 & 3.47 & 3.59\\
%           &{\scriptsize \color{blue} +1.19\%} & {\scriptsize \color{blue} +6.14\%} &  {\scriptsize \color{blue} +15.74\% }& {\scriptsize \color{blue} +20.97\%} & {\scriptsize \color{blue} +34.35\%} & {\scriptsize \color{blue} +11.72\%} & {\scriptsize \color{blue} +7.7\%} & {\scriptsize \color{blue} +8.88\%}\\
%         D-ULD++ (K=10) & \textbf{2.19} & \textbf{2.78} &  \textbf{2.92} & \textbf{3.62} & \textbf{2.12} & \textbf{2.85} & \textbf{2.89} & \textbf{3.12}\\
%         & {\scriptsize \color{blue} +31.34\%} & {\scriptsize \color{blue} +34.28\%} & {\scriptsize \color{blue} +50.91\%} & {\scriptsize \color{blue} +54.52\%} & {\scriptsize \color{blue} +59.31\%} & {\scriptsize \color{blue} +39.23\%} & {\scriptsize \color{blue} +23.13\%} & {\scriptsize \color{blue} +20.81\%}\\
%     \end{tabular}
%     \caption{Error comparison on MAFL, AFLW, LS3D and CatHeads, in Forward and Backward NME (denoted as F and B). The
% results of other methods are taken directly from the papers (for the case where all MAFL training images are used to train
% the regressor and the error is measured w.r.t. to 5 annotated points).  Where possible, we used pre-trained models, otherwise
% we re-trained these methods using the publicly available code. A set of 300 training images is used to train the regressors.
% Error is measured w.r.t. the 68-landmark configuration typically used in face alignment. The best performance is in \textbf{bold}.  Below ZeroShot and D-ULD++ are the (relative) percentage improvements over the best published results shown underlined.}
%     \label{tab:results}
% \end{table*}

% \begin{table}[h]
% \small
%     \centering
%     \begin{tabular}{ccccc}
%     \textbf{Method} & \multicolumn{2}{c}{\textbf{AFLW}} & \multicolumn{2}{c}{\textbf{MAFL}}\\
%           & F & B & F & B\\
%                   \hline
%          ZeroShot & 
%          4.98 & 6.29 & 3.14 & 3.98\\
%          D-ULD & 3.42 & 4.89 & 2.82  & 3.21  \\
%          + PP  &  3.15 & 4.46 & 2.68 & 3.12\\
%          + (TSC w/ Full VAE) & 3.07 & 4.12 & 2.59 & 3.03 \\
%          + TSC (D-ULD++) &  \textbf{2.92} & \textbf{3.62} & \textbf{2.19} & \textbf{2.78}\\
%     \end{tabular}
%     \caption{Ablation Evaluation on AFLW and MAFL. PP stands for pose-guided proxy task and TSC stands for two-stage clustering. }%F and B stand for forward and backward NME\%.}
%     \label{tab:ablation}
% \end{table}

% \begin{table}[h]
%     \scriptsize
%     \centering
%     \begin{tabular}{ccccc}
%        \multirow{2}{*}{\textbf{Methods}}  & \multicolumn{2}{c}{\textbf{MAFL}} & \multicolumn{2}{c}{\textbf{AFLW}} \\
%          & Sil. & CH & Sil. & CH\\
%          \hline 
%       ZeroShot ($K=30$)  & 0.74 & 357.4 & 0.72  & 142.9\\
%       D-ULD ($K10$)  & 0.79 & 372.1 & 0.81  & 182.3\\
%       D-ULD ($K=30$)   & 0.82 & 382.6 & 0.83  & 190.7\\
%       D-ULD++ ($Q=10,K=10$)  & 0.86 & 377.4 & 0.86  & 192.3\\
%       D-ULD++ ($Q=10,K=30$)   & 0.87 & 392.6 & 086  & 194.7\\
%     \end{tabular}
%     \caption{Quality of clustered landmark representations %for ZeroShot, D-ULD and D-ULD++ 
%     using Silhouette coefficient (Sil.) and Calinski-Harabasz (CH) Index. $Q$ and $K$ are the number of pose 
%  and  keypoint clusters.}
%     \label{tab:clustering-coefficients} \vspace{-0.5em}
% \end{table}

% % \begin{figure}[h]
% %     \centering
% %   \subfloat[ ]{\includegraphics[width=0.21\textwidth]{./figs/mafl_num_clusters.pdf}
% %     \label{fig:mafl-num-clusters}}
% %   \subfloat[]{
% %    \includegraphics[width=0.21\textwidth]{./figs/aflw_num_clusters.pdf}
% %     \label{fig:aflw-num-clusters}
% %   }
% %   \caption{Impact of number of clusters on performance. Along the X-axis and Y-axis number of clusters for keypoints and poses are shown respectively. For each permutation of number of clusters the forward and backward NME is shown as a tuple.}
% %   \label{fig:cluster-impact}
% % \end{figure}


% \subsection{Results}
% \Cref{tab:results} summarizes the results of our approach and baselines. The simple ZeroShot baseline outperforms previously published methods across all datasets, notably surpassing them by over $30\%$ on LS3D and $10\%$ on AFLW for both forward and backward NME respectively.  This emphasizes the efficacy of Stable Diffusion features.
% %, which is unsurprising given that earlier methods depended on less expressive backbone networks. Further, the results of ZeroShot argue for a re-orientation of unsupervised landmark detection and related tasks from more complex architectures and training schemes towards exploring more effective ways to utilize existing the feature representations of pre-trained large models.
% %
% The interesting comparison is between Mallis (D) and D-ULD++. 
% %as both methods have common network features  and a two-stage self-training based supervision, with similar intitial stages. 
% %The key difference in both methods is the second stage of self-training based supervision. 
% Mallis (D) simply oversegments the initial clusters into more fine-grained clusters (the initial $K$ clusters are segmented into $M>>K$ clusters), while D-ULD++ proposes a pose-guided proxy task and a two-stage clustering.
% %
% The D-ULD++ outperforms Mallis (D) by notable margins (more than 20\% over published methods) on all four datasets. %This performance is achieved without any fine-tuning of the Stable Diffusion network. 

% %As can be clearly seen, D-ULD++ significantly outperforms the other methods margins of more than $50\%$ on LS3D, MAFL and AFLW. It also performs $30\%$ better than competing methods on CatHeads. The main reason for this is, the features we use are trained on much greater quantities of data and are thus more expressive.

% %We quantified the impact of these features using a zero-shot model (denoted ZeroShot in~\Cref{tab:results}) by randomly selecting keypoints from dataset images, extracting features from a pre-trained Stable Diffusion model, and clustering them with $K$-Means. For each image, we retained the closest descriptor to each cluster centroid along with its associated keypoint. As can be clearly seen, even a simple Zero-shot baseline improves upon previous results by a margin of above $X\%$ for all datasets. Adding our proposed self-training scheme (Ours in~\Cref{tab:results}) only further improves upon previous methods. We believe this sets a new paradigm for unsupervised landmark detection as the features from these networks achieve results far exceeding previous methods.  This highlights the emergent properties of training large models on vast amounts of data for image generation can also be utilized for tasks like unsupervised landmark detection with simple training schemes.

% \Cref{fig:ced-curves}  displays the Cumulative Error Distribution (CED) curves. %comparing various methods to D-ULD++. 
% Our D-ULD++ exhibits notably lower errors than the other methods. Further, compared to others, our method's curve displays a gradual slope, suggesting a gradual decline in keypoint localization accuracy. %In contrast, the curves for other methods start with higher base errors and exhibit steeper slopes, indicating a more abrupt decrease in landmark localization accuracy.
% %
% %\Cref{fig:qual-results} provides a visual comparison of landmarks discovered by D-ULD++ and various baselines on images across an almost $180^\circ$ pose range. % Jakab and Zhang completely fail to model large viewpoint changes learning mostly random landmarks in uniform areas and not repeatable edges. Mallis manages to accurately detect a few keypoints across the poses like the lip edges,  but fails on other keypoints. This is probably due a combination of the poorer Stage2 self-training than D-ULD++, as well as less expressive features. D-ULD++ is to reliably keypoints across $180^\circ$ pose variations.
% %
% \Cref{fig:hungarian-plot} gives further insight into the localization accuracy and reliability of the landmarks detected by D-ULD++. In MAFL, which has for each image 68 facial landmarks across the various facial regions, each landmark is aligned with the best-matching unsupervised landmarks using the Hungarian algorithm. A value of $K=30$ is employed across all methods. Notably, our detected landmarks exhibits a high level of accuracy in tracking semantically relevant facial landmarks. D-ULD++ has almost perfect accuracy in detecting keypoints in the eyebrow, nose, eyes and mouth region.


% %To further demonstrate that, we evaluate how accurately raw unsupervised landmarks track supervised landmark locations in Fig. 8.


% % \begin{figure}
% %     \centering
% %     \includegraphics[height=0.32\textwidth]{./figs/compiled.pdf}
% %     \caption{Comparison of landmarks discovered by various methods across the various poses on LS3D. }
% %     \label{fig:qual-results} \vspace{-1em}
% % \end{figure}

% % \subsection{Pose Analysis}
% % We use a trained pose regressor to quantify whether 


% \section{Ablation and Analysis}
% \label{sec:ablation}

% \noindent\textbf{Performance contribution of our different methods:} Over ZeroShot baseline, our D-ULD algorithm provides consistent improvement in both forward and backward NME (\Cref{tab:ablation}). Upon introducing pose-guided proxy task (PP) in D-ULD, we see a further improvement in all instances. Finally, after including our two-stage clustering (TSC) with PP in D-ULD, we note a consistent notable improvement over each of the variants. Further to assess the contribution of 

% %\noindent\textbf{Two-stage clustering:} ~\Cref{tab:ablation} compares our two-stage clustering (TSC) in D-ULD++ with simple clustering in D-ULD. We see that, our TSC mostly improves over simple clustering variants in both clustering quality metrics i.e. Silhouette coefficient and Calinski-Harabasz (CH) Index.
% %We provide the performance contribution of our basel in ~\Cref{tab:ablation} first reports the performance of ZeroShot a

% % \noindent\textbf{Effect of Keypoint Self-Training:}  %Over the ZeroShot method in~\Cref{tab:results} we assess the overall impact of the keypoint pseudo-label based self-training. 

% % While ZeroShot does improve upon the previous SOTA by across all four datasets, on analyzing the NME breakup across different poses, shown in~\Cref{fig:method-quant} it is clear that it has a significantly lower error on front oriented faces as compared to the side profiles. This probably indicates that the training set used to train StableDiffusion has an over-representation of front-oriented faces. Frequently the faces generated with Stable Diffusion and similar methods are front-facing, perhaps indicating a bias to this orientation. 

% % Self-Training relies on a significant enough portion of the initial pseudo-labels to be accurate, so as to improve the classification accuracy for the entire dataset. As was shown in~\Cref{fig:method-qual}, certain keypoints like (lip corners, nose tip and iris) are reliably detected by ZeroShot. The D-ULD based self-training scheme is able to improve upon ZeroShot across the different pose variations by margins of over $20\%$  for forward and backward NME on AFLW and MAFL as shown in~\Cref{tab:ablation} and respectively by leveraging keypoint location consistency across viewpoints to bring the corresponding descriptors closer in feature space.
% \noindent\textbf{Effect of TSC based Self-Training:} 
% To get a better understanding of whether the pseudo-labels from two-stage clustering (TSC) do indeed capture pose variations, we do a simple cluster analysis. Recall D-ULD++ generates a latent pose code for each image landmarks, \ie there is a \emph{1-to-1} relation between the latent code and image landmarks. These latent codes are then clustered into $Q$ clusters. As the LS3D images come with the 5 yaw-angle ranges (the ranges are shown in~\Cref{fig:cluster-analysis}) they belong to, we cluster the latent codes into $Q=5$ clusters. Then for the latent codes within each cluster, we find to which yaw-angle range do the  majority of the latent codes belong to (by checking the range of their corresponding images) and map each cluster to a yaw-angle range. We find that the $Q=5$ clusters neatly map to each of the $5$ ranges. In the process, we also measure the percentage of latent codes that lie within the clusters assigned range. We refer to this percentage as the clustering accuracy $\%$. \Cref{fig:cluster-analysis} shows the cluster accuracy for $K=10$ clusters as a function of iterations for the various pose ranges. As can be clearly seen, clustering accuracy increases up to iteration $50k$ before levelling off. ~\Cref{tab:ablation} compares our two-stage clustering (TSC) in D-ULD++ with simple clustering in D-ULD. We see that, our TSC mostly improves over simple clustering variants in both clustering quality metrics i.e. Silhouette coefficient and Calinski-Harabasz (CH) Index.

% %maximum number of elements within the cluster fall into. This way we map each cluster to a single yaw-angle range. We compute 

% %$$ shows the percentage of the images within a cluster that lie within the same yaw ranges for LS3D. We show the yaw-angle range-wise split as well as overall accuracy. As the value of $Q$ is increased from $10$ to $30$, the overall accuracy $\%$ increases $XX\%$. Also, we show the accuracy $\%$ after various epochs. Pose pseudo-Label self-training improves the overall accuracy by $\%$ at epoch 30 with significant improvements for the more challenging side-profile ranges of $XX\%$ $XX\%$ , \ie $(-90^\circ,-60^\circ)$  and  $(60^\circ,90^\circ)$ respectively. 

% \begin{figure}[h]
%     \centering
% \includegraphics[scale=0.32]{./figs/clustering_accuracy.pdf}
%     \caption{Clustering accuracy percentages are reported across different yaw-angle ranges and overall for D-ULD++ on LS3D. The variable $I$ denotes the iteration number, as a multiple of 1000.}
%     \label{fig:cluster-analysis} \vspace{-1em}
% \end{figure}


% \noindent\textbf{Hyper-Parameter Study:}~\Cref{fig:cluster-impact} shows the effect of varying the number of clusters for $K$-Means on Forward and Backward NME for both keypoint and pseudo-pose clustering. We denote $K$ and $Q$ as the  number of clusters for keypoint and pseudo-pose clustering respectively. 
% %
% Increasing $Q$ and $K$ has the effect of lowering both NMEs. As $K$ increases the keypoints captured with each cluster are more specific and localized. Similarly, increasing $Q$ would have the effect of capturing finer pose variations. This saturates at $Q=30$ and $K=30$, but this maybe due to the limitation of the dataset size.

% \begin{figure}[!htp]
%     \centering
%   \subfloat[ ]{\includegraphics[width=0.24\textwidth]{./figs/mafl_num_clusters.pdf}
%     \label{fig:mafl-num-clusters}}
%   \subfloat[]{
%    \includegraphics[width=0.24\textwidth]{./figs/aflw_num_clusters.pdf}
%     \label{fig:aflw-num-clusters}
%   }
%   \caption{Impact of number of clusters on performance. Along the X-axis and Y-axis number of clusters for keypoints and poses are shown respectively. For each permutation of number of clusters the forward and backward NME is shown as a tuple.}
%   \label{fig:cluster-impact}
% \end{figure}


% \section{Conclusion}
% \label{sec:conclusion}
% We explored the effectiveness of stable diffusion to tackle  unsupervised landmark detection (ULD) problem. We first proposed a ZeroShot baseline that is only based on clustering of diffusion features and nearest neighbour querying that excels in performance than SOTA methods. This motivated us to develop a ULD algorithm using diffusion features (D-ULD) which turns out to be an excellent algorithm. We further build on D-ULD to propose a pose-guided proxy task and a two-stage clustering mechanism as D-ULD++. Our methods achieve significant improvement over existing SOTA methods.


% % Leveraging the remarkable power of diffusion models, we propose a novel self-training based scheme for unsupervised discovery of landmark objects. 

% % We presented a novel path for unsupervised discovery ofobject landmarks based on two ideas, namely self-training and recovering correspondence. The former helps our system improve by using its own predictions and constitutes a natural fit for training an object landmark detector starting from generic, noisy keypoints. The latter, although being a key property of object landmarks detectors, has not been previously used for unsupervised object landmark discovery. Compared to previous works, our approach can learn view-based landmarks that are more flexible in terms of changes in 3D viewpoint, providing superior results on a variety of challenging facial and human pose datasets.



==> sec/method.tex <==

% %%%%%%%%% BODY TEXT
% \section{Proposed Diffusion Based ULD Algorithm}
% \label{sec:method}

% Existing works targeting unsupervised landmark discovery struggle under various intra-class variations.
% %, for instance large out-of-plane rotations and self-occlusions. 
% In pursuit of overcoming these challenges, we intend to explore the potential of a recent class of self-supervised learning methods namely diffusion-based generative models \cite{ho2020denoising, song2020score,rombach2022high} for unsupervised landmark detection.
% %
% %The success of diffusion models in generating high-quality images, suggests that their internal representations contain meaningful cues which could be useful toward solving tasks other than image synthesis. Some recent works 
% %have used the representations of these pre-trained web-scale diffusion models like Stable Diffusion to achieve state-of-the-art performance in semantic correspondence tasks~\cite{luo2023diffusion, zhang2023tale, tang2023emergent}. 
% We first propose that a simple clustering of the fixed internal representations of the diffusion model, taken at random positions within object RoI. At inference, nearest neighbour querying is used to discover zero-shot landmarks (Sec.~\ref{subsection:Motivation: A Simple Clustering is all You Need}). %that outperforms existing works. 
% Motivated by excellent performance of zero-shot, we propose an unsupervised landmark detection algorithm (D-ULD) founded on diffusion features (Sec.~\ref{subsec:Stable Diffusion based ULD pipeline}). 
% %that uses self-training for pseudo-labels and clustering of keypoint descriptors for pseudo-labeling and emerges as a strong baseline (Sec.~\ref{subsec:Stable Diffusion based ULD pipeline}). %to learn correspondences across object images. 
% We further improve D-ULD by introducing a new pose-guided proxy task (Sec.~\ref{subsubsection:Pose-guided Proxy Task}).
% %harness the potential of this strong baseline by introducing a new pose-guided proxy task (Sec.~\ref{subsubsection:Pose-guided Proxy Task}). 
% It reconstructs landmarks after projecting them to a latent pose space. % 3D pose as latent codes. 
% To better capture the intra-class variations in landmark representations, we exploit this unsupervised latent pose space information to propose a two-stage clustering mechanism (Sec.~\ref{subsubsection:Two-stage Clustering mechanism}). After incorporating latent space-based proxy task and two-stage clustering mechanism in D-ULD, we contribute a new algorithm for unsupervised landmark discovery, dubbed as D-ULD++. ~\cref{fig:architecture_diagram} provides an overview of D-ULD and D-ULD++ algorithms.


% \noindent\textbf{Problem statement:} We assume the availability of a set of images  $\SX = \{\mathbf{x} \in \RR^{H \times W \times 3}\}$ of a specific object category e.g., faces. After learning an initial set of keypoints on $\SX$ via SILK~\cite{gleize2023silk}, our training set becomes $\SX = \{\mathbf{x_j}, \{\mathbf{p_i^j}\}_{i=1}^{N_j} \}$, where $\mathbf{p}_i^j \in \RR^2$ is a keypoint in 2D space and $N_j$ is the number of keypoints detected in image $j$. These learned keypoints don't necessarily correspond to ground truth landmarks. 
% %\textcolor{red}{More than one object landmark will not be part of $\mathbf{p_i^j}$}. 
% %Keypoints may cover many areas in an image, and could also include outliers. 
% Relying only on $\SX$, our aim to train a model $\Psi: \SX \rightarrow \SY$, where $\SY \in \RR^{H^o \times W^o \times K}$ is the space of output heatmaps representing confidence maps for each of the $K$ object landmarks we wish to detect \cite{mallis2023keypoints}.  %We further assume that, the structure of $\SY$ provides both order and landmark correspondence recovery.

% \noindent\textbf{Diffusion model overview:} Diffusion models are a class of generative models that approximate the data distribution by denoising a base data distribution (assumed Gaussian). In the forward diffusion process,  the input image \textbf{I} is gradually transformed into a Gaussian noise over a series of $T$ timesteps. %What is meant by Gaussian? Is it Gaussian noise?
% Then a sequence of denoising iterations $\epsilon_{\theta}(\mathbf{I}_t,t)$, parameterized by $\theta$, and $t = 1 \hdots T$ take as input the noisy image $\mathbf{I}_t$ at each timestep and predict the noise $\epsilon$ added at that iteration \cite{ho2020denoising}. %The diffusion objective is given by {:
% %\begin{equation}
% %    \mathcal{L}_{DM} = \mathbb{E}_{\mathbf{I},t,\epsilon \sim \mathcal{N}(0,1)}  \left[ || \epsilon - \epsilon_\theta(\mathbf{I}_t,t) ||_2^2  \right].
% %\end{equation}
% Latent Diffusion models (LDM)~\cite{rombach2022high}, instead of operating on images directly encode images  as latent codes \textbf{z} and perform diffusion process. A decoder maps the latent representation to the image again.  %The objective for an LDM is:
% \begin{equation}
%     \mathcal{L}_{LDM} = \mathbb{E}_{\mathbf{I},t,\epsilon \sim \mathcal{N}(0,1)}  \left[ || \epsilon - \epsilon_\theta(\mathbf{z}_t,t) ||_2^2  \right].
% \end{equation}
% The denoiser for LDM consists of self- and cross-attention layers~\cite{vaswani2017attention}. We make use of the features of a pre-trained Stable Diffusion LDM for our method \cite{rombach2022high}. % \ie \textcolor{red}{we use Stable Diffusion as frozen}. %This is not required.
% %We further input empty strings as text prompts, as our objective is to explore the use of diffusion features in a self-supervised manner for unsupervised landmark detection.


% % Our methods breaks down this problem into two main stages:
% % \begin{itemize}
% %     \item In the initial stage, self-training is used to learn correspondences between the learned keypoints across images of the dataset. This also serves to build a keypoint based representation for each image in $\SX$.
% %     \item In the second stage, the updated keypoints from the previous step are used to train a variational autoencoder (VAE). The generated latent codes from the VAE are then used for second level or pose pseudo-label self-training.
% % \end{itemize}

% % \noindent\textbf{Preliminaries:} Diffusion models are a class of generative models that approximate the data distribution by denoising a base data distribution (assumed Gaussian). In the forward diffusion process,  the input image \textbf{I} is gradually transformed into a Gaussian over a series of $T$ timesteps. Then a sequence of denoising iterations $\epsilon_{\Psi}(\mathbf{I}_t,t)$, parameterized by $\Psi$, and $t = 1 \hdots T$ take as input the noisy image $\mathbf{I}_t$ at each timestep and predict the noise $\epsilon$ added at that iteration. The diffusion objective is given by:

% % \begin{equation}
% %     \mathcal{L}_{DM} = \mathbb{E}_{\mathbf{I},t,\epsilon  \mathcal{N}(0,1)}  \left[ || \epsilon - \epsilon_\theta(\mathbf{I}_t,t) ||_2^2  \right]
% % \end{equation}

% % Latent Diffusion models (LDM)~\cite{}, instead of operating on images directly initially encode images \textbf{I} as latent codes \textbf{z}  and perform diffusion on this latent code. A decoder maps the latent representation to the image again.  The objective for an LDM is:

% % \begin{equation}
% %     \mathcal{L}_{LDM} = \mathbb{E}_{\mathbf{I},t,\epsilon  \mathcal{N}(0,1)}  \left[ || \epsilon - \epsilon_\theta(\mathbf{z}_t,t) ||_2^2  \right]
% % \end{equation}

% % The denoiser for LDMs consists of self and cross-attention layers~\cite{}. We make use of the features of a pre-trained Stable Diffusion LDM for our method, \ie we use Stable Diffusion as frozen. We further input empty strings as text prompts, as our objective is to explore the use of diffusion features in a self-supervised manner for landmark detection. 
% %\textcolor{red}{\noindent\textbf{Notation:} $j$,$j'$ are indices over the images in a dataset. $i$, $i'$ are indices over keypoints. $[K]$ denotes the set $\{1, \hdots, K\}$.}
% % This notaion is not required. 
% %\subsection{A Simple Clustering is All You Need}
% \subsection{Proposed Zero-Shot Baseline}
% \label{subsection:Motivation: A Simple Clustering is all You Need}
% %\noindent\textbf{Motivation:} %Recent works ~\cite{luo2023diffusion, zhang2023tale, tang2023emergent} have shown the internal representations of diffusion models e.g., stable diffusion are useful for tasks beyond image synthesis, such as semantic correspondence. 
% %It has recently been found that  features from diffusion models are effective for the task of semantic correspondence~\cite{luo2023diffusion, zhang2023tale, tang2023emergent}.  It signifies that these generative models understand the underlying semantics of common objects. Motivated by this, 
% \noindent We propose a zero-shot baseline to measure the efficacy of diffusion features for the task of unsupervised landmark detection comprised of feature aggregation, clustering and exemplar assignment. %Below, we describe the methodology for our zero-shot baseline.


% %Motivated by this, we first developed a simple baseline to measure the efficacy of these diffusion features for the task of unsupervised landmark detection. We use a frozen Stable Diffusion models as our feature extractor. 
 

% \noindent\textbf{Feature aggregation:} Feature maps in diffusion models are spread out over network layers and diffusion time-steps. So, extracting useful feature descriptors from them is a non-trivial task. Similar to the recent works~\cite{luo2023dhf,hedlin2023unsupervised}, we  employ a network that aggregates features over layers and time-steps to obtain a  single feature map.
% %
% The aggregator network, takes as input the features maps $\mathbf{r}_{l,t}$  obtained from Stable Diffusion for an input image $\mathbf{x}_j$. We upscale $\mathbf{r}_{l,t}$ to image resolution and pass it through a bottleneck layer $\mathbf{B}_l$~\cite{he2016deep,xu2023open} to obtain a fixed channel count, and weight it with a mixing weight $\mathbf{w}$. The final aggregated feature map is given by: %confirm the lefthand side
% \begin{equation}
%  {F_{ag}=}   \sum_{t=1}^{T} \sum_{l=1}^{L} \mathbf{w}_{l,t}\mathbf{B}_l(\mathbf{r}_{l,t}), \mathrm{SD}(\mathbf{x})=\{\mathbf{r}_{l,t}\}_{l=1,t=1}^{L,T}
%     \label{eqn:feat-aggr}
% \end{equation}
% where $L$ is the number of layers, $T$ is the number of timesteps. %$l$ and $t$ are layer and time indices, respectively. 
% %Bottleneck layers are shared across timesteps %giving $L$ in total 
% %to maintain a constant feature dimension. %across layers.
% There are $L \times T$  combinations of layer indices and timesteps. We learn unique mixing weights $\mathbf{w}_{l,t}$ across all layer and timestep combinations via backpropagation. %We denote the aggregator network as $\Psi_{b}$ which is a pre-trained network of~\cite{luo2023dhf}. 
% The overall process of getting feature map $\mathbf{F}_{ag}$ may be defined as: $\mathbf{F}_{ag}=\Psi_b(\mathbf{x})$, where $\Psi_b$ includes both the stable diffusion process and the feature aggregation. %The output feature map from $\Psi_{b}$ have $128$ channels. %From henceforth on, when referring to feature extraction, we specifically mean extraction from the aggregator network. %loss function of aggregator?

% \noindent\textbf{Clustering:} 
% For every image in the training set, we randomly sample pixels within the ROI region in the output feature map $F_{ag}$. For each sampled pixel, we get a descriptor which is then clustered using k-means and the cluster centroids from the training set are retained. For the detection of ROI, pretrained Detectron~\cite{wu2019detectron2} is employed.
% %The first step toward constructing this baseline involves randomly sampling pixels within the image ROI (e.g., human and cat faces), and extracting their corresponding descriptors from $\Psi_b$. %Why randomly sampling? Why not key points referred previously?
% %Such features are extracted for every image of the training set. In the second step, they are clustered via K-Means and the cluster centroids from the training set are retained. 
% On the test set, again random pixels are sampled for each image within ROI, and after their corresponding descriptors are extracted, they are assigned the label of their closest  cluster. Each image then may consist of multiple pixel locations belonging to a particular cluster. %Each cluster can thus have multiple keypoints associated with it per image. 
% As some of these can be noisy assignments, we prune the locations so that per image each cluster has a single best location. We do this via  {exemplar assignment}.

% \noindent\textbf{Exemplar assignment:} We assign to each image at most $K$ pixel locations by choosing for each cluster the locations whose descriptor is closest to the cluster centroid in feature space. We discard the remaining locations, leaving for each image at most $K$ pixel locations. These $K$ pixel locations after assignment are considered as discovered landmarks. 

% %(some clusters may have no keypoints in an image). %How zero assignment is decided? Threshold? 
% %\textcolor{red}{Since this set of operations is referenced multiple times, we opt for the shorthand \emph{exemplar assignment} to simplify communication.}
% % This sentence is not required. 
% %  refer to this set of operations multiple time 
% %The exemplar assignment completes our zero-shot baseline  dubbed as ZeroShot.
% %method is referred to as ZeroShot in our experiments
% % On the test set, we randomly sample keypoints for each image, and after extracting their corresponding descriptors, we assign them label by finding  assigned 
% % extracted and assigned the label of their closest corresponding cluster. 
% % This method is referred to as ZeroShot in our experiments. 

% \noindent\textbf{Analysis:} %\Cref{tab:results} shows the results of ZeroShot on the four different datasets. \emph{This simple baseline outperforms previous approaches without any training by margins of $7-10\%$ across all four datasets.} 
% %
% \Cref{fig:method-qual} shows some qualitative results of ZeroShot on the AFLW dataset. While ZeroShot is able to reliably detect keypoints for most front-oriented faces, it occasionally tends to confuse keypoints on the left and right side of side-oriented faces for some examples. Further, it tends to have poor keypoint localization on side profile faces. To better understand the method we take a more fine-grained look at the results.
% %
% \Cref{fig:method-quant} shows the forward and backward NME\% for ZeroShot  amongst other methods for various yaw angles on the AFLW dataset. Errors for the front-facing angles $(-30^{\circ} \text{ to } 30^{\circ})$ are significantly lower than those of the more side-oriented ones. Compared to \cite{mallis2023keypoints}, an error reduction of $14.6\%$ in  front-oriented faces is seen. Whereas a more modest improvement of $4.5\%$ is seen for side-oriented faces (yaw angles $(-60^\circ \text{ to }-30^\circ)$ and $(30^\circ \text{ to }60^\circ)$) and $2.1\%$ for more extreme view points (yaw angles $(-90^\circ \text{ to }-60^\circ)$ and $(60^\circ \text{ to }90^\circ)$). %We show additional analysis of ZeroShot in~\Cref{sec:experiments} on the LS3D Dataset. %We also provide additional per-keypoint localization accuracy analysis for ZeroShot in the supplementary. 
% %
% %To measure per-keypoint localization accuracy, we make use of the ground-truth keypoints provided by the LS3D dataset. This dataset consists of face images, each annotated with 68 keypoints. We take from a training set image $\mathbf{x}_j$, a ground-truth keypoint $\mathbf{p}^j_i$. In a test image $\mathbf{x}_{j'}$, we find it's corresponding keypoint $\mathbf{p}^{j'}_i$ by a nearest neighbor assignment in the feature space between the descriptor of $\mathbf{p}^j_i$ and the  descriptors of the keypoints of $\mathbf{x}_{j'}$ . We then compute the pixel distance between $\mathbf{p}^{j'}_i$ and the ground truth keypoint in $\mathbf{x}_{j'}$ corresponding to $\mathbf{p}^j_i$, denoted as $\overline{\mathbf{p}}^{j'}_i$. This distance $||\mathbf{p}^{j'}_i-\overline{\mathbf{p}}^{j'}_i||$ is measures how accurately the keypoints are localized.
% %Using the keypoints obtained in the test set images by ZeroShot
% The limitations of ZeroShot motivate our next contribution.% where we propose an unsupervised landmark detection (ULD) algorithm based on diffusion features (D-ULD); it leverages pseudo-labeling of keypoints via descriptor clustering and self-training with the constructed pseudo-labels.

% %propose to iteratively alternate
% %between pseudo-labelling of keypoints  via descriptor clustering, and
% %model self-training with the produced pseudo-labels. 

% %\subsection{Keypoint Self-Training} 

% \subsection{Proposed  Diffusion based D-ULD Algorithm} 
% \label{subsec:Stable Diffusion based ULD pipeline}

% \noindent In this section, we describe our unsupervised landmark detection algorithm (D-ULD) based on diffusion features that uses clustering to obtain pseudo-labels (PLs) and employs these PLs for self-training.


% \noindent\textbf{Network Structure:} We append a descriptor head $\Psi_f$  and a landmark detector head $\Psi_d$ after $\Psi_b$. 
% %Using the feature map $F_{ag}$ obtained from $\Psi_b$, we append  a descriptor $\Psi_f$ and a detector $\Psi_d$. 
% %
% The detector head $\Psi_d$ will produce a single-channel heatmap $\mathbf{H}_j = \Psi_d(\Psi_b(\mathbf{x}_j)) \in \mathbb{R}^{H \times W \times 1}$ for image $\mathbf{x}_j$. This heatmap reveals the confidence of the model for an object landmark at a given location. Non-maximum suppression is used to obtain landmarks from $\mathbf{H}_j$ \cite{mallis2023keypoints}. The descriptor $\Psi_f$ produces for image $\mathbf{x}_j$ a descriptor volume $\mathbf{F}_j = \Psi_f(\Psi_b(\mathbf{x}_j)) \in \mathbb{R}^{H \times W \times D}$, where $D$ is the feature dimension. From $\mathbf{F}_j$, we extract a feature descriptor $f_i^j \in \RR^D$ corresponding to the landmark location found by $\Psi_d$.  We denote the network consisting of $\Psi_b$, $\Psi_f$ and $\Psi_d$  as $\Psi$.

% \noindent\textbf{Bootstrapping:} We initially train the network $\Psi$ (except stable diffusion network) via a self-supervised keypoint training scheme~\cite{gleize2023silk}. %Our objective is to improve on the random pixel locations used in ZeroShot baseline, by learning dataset specific keypoints.
% %
% Specifically, during bootstrapping the network $\Psi$ is trained by learning correspondences between an image and it's augmentation, by minimizing a BCE loss for the detector head $\Psi_d$ and a negative-log-likelihood loss for the descriptor head $\Psi_f$. We use flips and random rotations as augmentations. After the initial keypoint learning, 
% the training set consists of images, learned keypoints and the corresponding descriptors, \emph{i.e.} $\SX = \{\mathbf{x_j}, \{\mathbf{p^j_i},\mathbf{f^j_i}\} \mid i \in \text{keypoints for image} \ \mathbf{x}_j  \}$.

% \noindent\textbf{Self-Training:}
% To improve landmark detection across a larger spectrum of viewpoint changes and symmetric view pairs, we resort to a self-training scheme that uses keypoint pseudo-labelling \cite{mallis2020unsupervised}.
% %
% %use a keypoint pseudo-label based self-training scheme.
% %
% We initialize this step by clustering all keypoint descriptors $\{ \mathbf{f}^j_i \mid \forall i \in \text{keypoints in } \mathbf{x}_j, \forall j \in \text{images}\}$ into $K$ clusters using $K$-means. Then, we perform exemplar assignment and remove redundant keypoints, leaving for each image $\mathbf{x}_j$ a set of $K$ keypoints and their corresponding descriptors $\{\mathbf{p}^j_i,\mathbf{f}^j_i \mid \forall i \in \{1, \hdots, K\} \}$. This provides us with a pseudo-label $\mathbf{c}^j_i  \in \{1, \hdots K\}$ for keypoint $\mathbf{p}^j_i$. % $\mathbf{c}^j_i \in \{1, \hdots K\}$ denotes the pseudo-label for $\mathbf{p}^j_i$.
% %
%  %we also remove redundant keypoints for image $x_j$ by only retaining a single descriptor per cluster for each image. For a given image $j$, we find for each
% %cluster $k$, from keypoints $\{\mathbf{p}^j_i \mid \forall i \in \text{image j}\}$ the 
% % descriptor closest to the centroid and remove duplicate occurrences of the same
% %cluster label $k$. Thus for each image $\mathbf{x}_j$ there are a set of $\leq K$ keypoints as some clusters may not occur in an image. 
% %
% Updating the training dataset with pseudo-labels, our dataset is now $\SX = \{\mathbf{x}_j, \{\mathbf{p}^j_i,\mathbf{f}^j_i,\mathbf{c}^j_i  \}_{i=1}^{K} \}$. 

% %$\mathbf{c}^j_i \in \{1, \hdots K\}$ denotes the pseudo-label for $\mathbf{p}^j_i$. %Without loss of generalization we assume all clusters are present while missing clusters for an image  will  be ignored without changing the formulation.
% %
% %Keypoint pruning also provides us keypoint correspondences across images of the training set, as for each $\mathbf{p}^j_i$ for image $i$, there exists at most one keypoint $\mathbf{p}^{j'}_{i'}$ in image $j'$ with the same cluster label, \ie $\mathbf{c}^{j}_{i} = \mathbf{c}^{j'}_{i'}$.
% %We exploit these cluster labels as landmark pseudo-label correspondences in our self-training scheme. 

% %
% %As every cluster has a representative keypoint in each image, this also provides correspondences across images which we intend to exploit for our self-training scheme.

% % \begin{figure}
% %     \centering
    
% %     \caption{Comparison of Forward and Backward errors (as NME \%) split by yaw-angles ranges on the AFLW~\cite{koestinger2011annotated} dataset for our method, the Zero Shot baseline with comparison to Mallis~\cite{mallis2023keypoints}.}
% %     \label{fig:method_nme}
% % \end{figure}

% \begin{figure}
%   \centering
%     \subfloat[]{
%     \centering
%     \includegraphics[width=0.42\textwidth]{figs/overall_method_qual.pdf}
%     \label{fig:method-qual}
%   }\newline
%   \subfloat[]{    \includegraphics[width=0.42\textwidth]{./figs/method_nme.png}
%     \label{fig:method-quant}}
%   \caption{Comparisons of ZeroShot, D-ULD and D-ULD++. (a)Qualitative results on exemplar images showing. Different colored keypoints 
%   (b) Yaw angle split of forward and backward errors  (as NME \%) for the AFLW~\cite{koestinger2011annotated} dataset. \cite{mallis2023keypoints} is shown for additional comparison.}
%   \label{fig:mainfig} \vspace{-1em}
% \end{figure}
% \noindent\textbf{Training objectives:} We use the pseudo-labels $\mathbf{c}^j_i$ contained in the training set $\SX$ to train the network $\Psi$.
% %After the initial clustering and image keypoint assignment step, each image $\mathbf{x}_j$ has associated with it a set of keypoints $\{ \mathbf{p}^j_i \mid j \in \text{images}, \ i \in  \text{keypoints for image} \ j \}$ and pseudo-labels $\mathbf{y}_j$. 
% %The network $\Psi$ consisting of the aggregation network $\Psi_b$, detector $\Psi_d$ and descriptor heads $\Psi_f$, is now trained using these pseudo-labels. 
% The loss corresponding to the detector head is the standard mean-squared error (MSE) loss between the pseudo-label heatmaps and detector head output. %Here the heatmap $G$ for a given image $\mathbf{x}_j$ is formed by placing 2D-Gaussian maps on each of
% To train the descriptor head $\Psi_f$, we use a contrastive loss that pulls feature descriptors  $\mathbf{f}^j_i$ from the same cluster together and pushes features from different clusters away from each other.
% %
% Once the training is done for a fixed number of epochs, the training set is updated with improved keypoints, descriptors, and new pseudo-labels. Thus,  $\mathbf{p}$, $\mathbf{f}$ and $\mathbf{c}$ are functions of the epoch $t$. We refer to the training set at epoch $t$ as $\SX_t = \{\mathbf{x}_j, \{\mathbf{p}^j_i(t), \mathbf{f}^j_i(t), \mathbf{c}^j_i(t) \}_{i=1}^K \}$.
% %

% % :
% % \begin{equation}
% %     \SL_{d} = ||G(\mathbf{x}_j) - \Psi_d(\Psi_b(\mathbf{x}_j)) ||^2
% %     \label{eqn:mse-detector}
% % \end{equation}

% % Here the ground-truth heatmap $G$ for a given image $\mathbf{x}_j$ is formed by placing 2D-Gaussian maps on each of
% % the keypoint locations.
% %
% % To train the descriptor head $\Psi_f$, we use a contrastive loss that pushes features from the same cluster together. Let $\mathbf{p}^j_i$ and $\mathbf{p}^{j'}_{i'}$ be two keypoints indexed by $i$ and $i'$ for images $j$ and $j'$ respectively. The loss we minimize to train $\Psi_f$ is:

% % \begin{eqnarray}
% %     \SL_f(\mathbf{x}_i^j,\mathbf{x}_{i'}^{j'}) = \mathbf{1}_{[\mathbf{c}^{j'}_{i'} = \mathbf{c}^{j}_{i}]} ||\mathbf{f}^j_i - \mathbf{f}^{j'}_{i'} || + \nonumber \\ \mathbf{1}_{[\mathbf{c}^{j'}_{i'} \neq \mathbf{c}^{j}_{i}]}\text{max}(0,m-||\mathbf{f}^j_i-\mathbf{f}^{j'}_{i'}|| \label{eq:desc-loss}
% % \end{eqnarray}

% % where recall $\mathbf{f}^j_i = \Psi_f(\Psi_b(\mathbf{x}_j))$ is the feature descriptor extracted at image $j$ for keypoint $\mathbf{p}^j_i$,. A margin $m$ is used to enforce
% % features corresponding to negative pairs to be far apart.  Our choice of positive pairs is obvious, as $\mathbf{c}^{j'}_{i'} = \mathbf{c}^{j}_{i}$ for only a single pair of keypoints in any two images. For negative pair selection, for a particular keypoint location $\mathbf{p}^j_i$ we pick $\mathbf{p}^{j'}_{i'}$ to be the farthest point by pixel distance for which $\mathbf{c}^{j'}_{i'} \neq \mathbf{c}^{j}_{i}$ holds.

% \noindent\textbf{Analysis:} \Cref{fig:method-quant}  shows across all yaw angles, our D-ULD algorithm improves the results significantly over ZeroShot. %Especially in the yaw-angle ranges $(-60^{\circ},-30^{\circ})$ and $(30^{\circ},60^{\circ})$ D-ULD improves upon ZeroShot by $\mathbf{XXX}$. 
% In~\Cref{fig:method-qual} for D-ULD, landmarks on the eye pupils, nose and mouth are accurately localized while the landmarks around the  eyes need further improvement. %For example, the blue landmark  around the eye region in the center two images and on the forehead region in the two side images. 

% \subsection{ Proposed D-ULD++ Algorithm} 
% \label{subsec:D-ULD++}

% While D-ULD algorithm improves upon the ZeroShot baseline across pose variations, it still has a tendency to output semantically non-meaningful landmarks for extreme poses.  It is because the landmark descriptors inherently contain local image information, and there is no explicit mechanism in the D-ULD to capture the collective spatial configuration of landmarks. To this end, we design a simple proxy task that takes the predicted landmark heatmaps from D-ULD and aims to reconstruct them after projecting into a low dimensional latent pose space. Next, to better capture the variations caused by large viewpoint changes, we propose two-stage clustering mechanism.


% \subsubsection{Pose-guided Proxy Task}
% \label{subsubsection:Pose-guided Proxy Task}
% % While our ULD pipeline is capable of improving the landmark detection across pose variations, it still has a tendency to learn semantically non-meaningful landmarks for more extreme variations.  This is because keypoints inherently contain local information image information. To handle these extreme pose variations, we propose to learn an image level representation of these learned keypoints via a proxy task, that we subsequently use to inject some pseudo-pose information via a two-stage clustering scheme~\Cref{sec:two-stage}.
% %Previous works have explored using the set of predicted keypoints from a network to detect poses~\cite{} for human pose estimation. We propose a similar proxy task, to learn image level representations from the predicted keypoints. 

% A relationship between the  facial landmarks and the corresponding pose of that face is quite intuitive. For example, the visibility of particular landmarks can be easily associated with a particular pose. Thus each pose constraints the landmark visibility and location to a relatively smaller space while each set of landmarks constraint the facial pose as well. Given accurate pose and landmark positions, a mapping may be learned in both directions. However, in our case, the pose supervision  is not available while the landmark positions are noisy. We therefore propose a proxy task to project the noisy landmarks to a latent pose space and then back project to the original space with the aim of removing the localization noise in landmarks.  
% Such a proxy task will constrain the collective configuration of land marks with respect to each other.

% %Our goal is to design a proxy task that is tightly connected to the task of landmark detection. In other words, while communicating with the landmark detector, it can encode the landmark configuration, possibly exhibiting several variations, as a shape information of a deformable object. In pursuit of this, we map the predicted landmarks to a latent pose code embedding and then reconstruct the original predicted landmarks from this latent code embedding. We realize this as a variational auto-encoder (VAE) denoted as $\Psi_V$. This $\Psi_V$ is appended to our descriptor head $\Psi_d$.

% %To this end, we  append a variational auto-encoder (VAE) denoted as $\Psi_V$ to our  descriptor head $\Psi_d$.
% %Assuming the input to the network $\Psi$ is image $\mathbf{x}_j$ and the predicted output heat map by the detector head $\Psi_d$ is $\mathbf{H}_f^j$, \ie $\mathbf{H}_f^j = \Psi_d(\Psi_b(\mathbf{x}_j))$.
% % 

% For this purpose we append an encoder-decoder network $\Psi_V$ to the descriptor head $\Psi_d$. The input to $\Psi_V$ is predicted landmark heatmap $\mathbf{H}_j$. $\Psi_V$ is trained to construct a pseudo ground-truth heatmap $\mathbf{G}^j$ formed by placing $K$ 2D-Gaussians corresponding to predicted landmark locations $\{ \mathbf{p}^j_i \mid i \in [K]\}$ on a single channel.
% %
% %on a single channel on each of the predicted landmark locations $\{ \mathbf{p}^j_i \mid i \in [K]\}$. 
% %
% The output of the encoder produces a latent pose code $\varphi_j$ corresponding to $\mathbf{H}_j$. 
% %as the latent code $\mathbf{l}_j \in \mathbb{R}^{3}$.
% This latent code is then used by the decoder to reconstruct the $\mathbf{G}_j$. %The $\Psi_V$ consists of residual blocks with \texttt{BatchNorm}-\texttt{LeakyRelu}-\texttt{Conv} blocks for the encoder and decoder. 
% The dimension of the latent vector is fixed to 64. The training loss for the this encoder-decoder architecture is the standard ELBO loss~\cite{kingma2013auto}. 
 
% \noindent\textbf{Discussion:} The $\Psi_V$ is trained on only landmark information without any pose supervision. We observe in~\Cref{sec:experiments} in-spite this limitation, the latent codes obtained after training in-fact capture relevant pose information. A $K$-Means clustering of the latent codes is done and the clusters thus obtained contain images corresponding to the same pose-range. The additional supervision by  $\Psi_V$  improved both forward and backward NME error by $7.8\% $ and  $12.4\%$ on AFLW and $4.9\% $ and  $6.4\%$ on MAFL in~\Cref{tab:results}. %The more modest improvements in MAFL, in comparison to AFLW, can be attributed to more front-facing images in the dataset.
%  %We leverage this `pseudo-pose' in~\cref{subsubsection:Two-stage Clustering mechanism} to learn keypoints consistent across wider pose variations. 
 
%  %improve improve matching across images with greater pose variation, in the process improving  provide additional supervision for the network.


 



% %We propose as a proxy task training our a variational auto-encoder, to reconstruction the keypoint heat map predicted by $\Psi_d$. Once trained, we show the latent codes learned by the VAEs contain pose information in~\Cref{sec:results}. 


%  %The VAE is trained via a standard ELBO loss~\cite{kingma2013auto}. 
%  %Once trained, the VAE can predict keypoint heatmaps. 
 
%  %We show these predicted keypoint heatmaps give pose information. We show through analysis in the results section (\Cref{fig:aaa}) that the latent codes indeed represent poses by performing a K-Means clustering of the latent codes and the majority of the poses contained in the clusters are similar.

% \subsubsection{Two-stage Clustering} 
% \label{subsubsection:Two-stage Clustering mechanism}
% In realistic settings, deformable objects like faces can undergo large variations like extreme 3D rotations. A simple clustering of keypoint descriptors is restrictive in capturing such variations due to the inherently local nature of keypoint information \cite{mallis2023keypoints, awan2023unsupervised}. This poses a limitation in achieving a robust ULD method.
% %This inherent reliance on local information could present itself as a limitation in realizing a robust ULD pipeline.
% To overcome this, we devise a two-stage clustering (TSC) mechanism which exploits the pseudo-pose generated by our pose-guided proxy task. In particular, TSC leverages the latent code to  perform  stage-1 pose-based clustering. Next, in each pose-based cluster, we perform stage-2 clustering of keypoint descriptors from images that belong to the same stage-1 cluster. Thus, TSC essentially decomposes the problem of recovering landmark correspondence under large intra-class variations into two stages. Moreover, it allows us to leverage both local and image-level information by using the learned keypoint descriptors and latent codes. Such a scheme ensures reduced within cluster variations compared to the simple clustering. 

% % To improve landmark detections across wider pose variations we leverage both local and image-level information by using the learned keypoint descriptors and latent codes for self-training. 

% In TSC, in the first stage,  latent codes $\boldsymbol{\varphi}_j$ are divided into $Q$ clusters using $K$-means, and latent code labels $\boldsymbol{u}_j \in [Q]$ are assigned. In the second stage,   we perform a further $K$-means clustering of  collection of keypoint descriptors $\mathbf{f}$ from images belonging to the same pose-based clusters. The number of clusters in the second stage is the same as the number of landmarks $K$ to be detected in a particular dataset. Thus, the two-stage clustering provides us with a total of $Q \times K$ clusters. $[R] = [Q] \times [K]$ denotes the new label set.
% %
% With this TSC, for given image $\mathbf{x}_j$, we find the pseudo-label $\mathbf{c}^{j}_{i}$, by retaining for each cluster $r \in [R]$, the keypoint whose descriptor is nearest to the cluster centroid. We then update the training set with the latent codes $\boldsymbol{\varphi}_j$, their labels $\boldsymbol{u}_j$, as well as the more fine-grained keypoint labels $\mathbf{c}^j_i$ obtained from TSC.
% %the more fine-grained labels $\mathbf{c}^j_i$ generated from TSC, as well as the pose-labels obtained by clustering the latent codes denoted by $\{ \boldsymbol{u}_j \in [Q] \}$.
% $\SX=\{\mathbf{x}_j, \{\mathbf{p}^j_i,\mathbf{f}^j_i,\mathbf{c}^j_i  \}_{i \in [R]}, \boldsymbol{\varphi}_j, \boldsymbol{u}_j  \}$ is the updated dataset. Now, similar to D-ULD, we alternate between the clustering and using the resulting pseudo-labels for supervision.



% % add to the training set, the latent code pseudo-labels to the training set. Thus the training dataset now consists of $\SX = \{\mathbf{x_j}, \{\mathbf{p}^j_i, \mathbf{f}^j_i, \mathbf{c}^{j}_i\}, \boldsymbol{l}_j, \boldsymbol{u}_j \mid j \in \text{keypoints for image } j, j \in \text{images}  \}$, where $\boldsymbol{l}_j$ is the latent code corresponding to $\mathbf{x}_j$ and $\boldsymbol{u}_j$ is it's pose pseudo-label.
% %
% %Similar to D-ULD, we alternate between clustering and using the resulting pseudo-labels for supervision. However, now 


% %However, now in addition to the keypoint pseudo-labels we also do so for the pose pseudo-labels.

% \noindent\textbf{Training objectives:} D-ULD++ is trained in two steps. In first step, we backprop through $\Psi_v$ using ELBO loss. Similar to D-ULD, the detector head $\Psi_d$ is trained via the MSE loss with the pseudo-labels obtained using TSC, and the the descriptor head $\Psi_f$ is trained using the contrastive loss on keypoint descriptors $\mathbf{f}_i^{j}$. In the second step, we do not use the decoder and so the ELBO loss. The detector head is trained same as first step, while the descriptor head is kept frozen. Instead, we just use the encoder in $\Psi_v$ and backprop through it using the contrastive loss which encourages latent codes with the same labels to be close to each other: 
% \begin{align}
% \SL_d(\boldsymbol{\varphi}_j,\boldsymbol{\varphi}_{j'}) = \mathbf{1}_{[\boldsymbol{u}_j = \boldsymbol{u}_{j'}]} ||\boldsymbol{\varphi}_j - \boldsymbol{\varphi}_{j'} || + \nonumber \\ \mathbf{1}_{[\boldsymbol{u}_j \neq \boldsymbol{u}_{j''}]}\text{max}(0,m-||\boldsymbol{\varphi}_j-\boldsymbol{\varphi}_{j''}||)
% \label{eqn:latent-opt}
% \end{align}
% %where $\boldsymbol{\varphi}_j$ is the output of the VAE Encoder $\Psi_V^{Enc}$, \ie $\boldsymbol{\varphi}_j = \Psi_V^{Enc}(\Psi_d(\Psi_b(\mathbf{x}_j))$. 
% %We select any $\boldsymbol{\varphi}_{j'}$ and $\boldsymbol{\varphi}_{j''}$ such that $\boldsymbol{u}_j = \boldsymbol{u}_{j'}$ and $\boldsymbol{u}_j \neq \boldsymbol{u}_{j'}$ respectively.



% % First, we train $\Psi_v$ using ELBO loss, next we only backprop through the encoder with our contrastive loss formulation. The detector head $\Psi_d$ is trained via the MSE loss with the pseudo-labels obtained using TSC. To train the descriptor head $\Psi_f$  contrastive loss is used encouraging latent codes with the same labels to be close to each other. We minimize the following loss:
% % \begin{align}
% % \SL_d(\boldsymbol{\varphi}_j,\boldsymbol{\varphi}_{j'}) = \mathbf{1}_{[\boldsymbol{u}_j = \boldsymbol{u}_{j'}]} ||\boldsymbol{\varphi}_j - \boldsymbol{\varphi}_{j'} || + \nonumber \\ \mathbf{1}_{[\boldsymbol{u}_j \neq \boldsymbol{u}_{j''}]}\text{max}(0,m-||\boldsymbol{\varphi}_j-\boldsymbol{\varphi}_{j''}||)
% % \label{eqn:latent-opt}
% % \end{align}
% % 


% %As in D-ULD, at a fixed number of epochs, the training set is refreshed with the network's output, including new keypoints, descriptors, cluster assignments, and latent code embeddings with their respective cluster assignments.


% \begin{figure*}
%     \centering
%     \includegraphics[scale=0.5]{./figs/Fig8.pdf}
%     \caption{Evaluation of the ability of raw unsupervised landmarks to capture supervised landmark locations on MAFL. Each unsupervised landmark is mapped to the best corresponding supervised landmark using the Hungarian Algorithm. Then accuracy is calculated for a distance threshold of $0.2\cdot$ $d_{iod}$ to a landmark location, where $d_{iod}$ is the interocular distance. Accuracy is shown for each of the 68-facial landmarks sorted by ascending order of index. Different landmark areas are highlighted with different colours and labelled as such (1-17 face contour, 18-27 eyebrows etc.}
%     \label{fig:hungarian-plot}
% \end{figure*}



% \begin{figure*}
%     \centering
%   \subfloat{
%   \centering
%     \includegraphics[width=0.95\textwidth]{./figs/legend.pdf}
%     \label{fig:legend-ced}}\newline
%   \subfloat{
%     \includegraphics[width=0.23\textwidth]{./figs/mafl_forward.pdf}
%     \label{fig:mafl-fwd}}
%   \subfloat{
%     \includegraphics[width=0.23\textwidth]{./figs//mafl_backward.pdf}
%     \label{fig:mafl-bwd}
%   }
%   \subfloat{
%     \includegraphics[width=0.23\textwidth]{./figs/ls3d_forward.pdf}
%     \label{fig:ls3d-fwd}
%   }
%   \subfloat{
%     \includegraphics[width=0.23\textwidth]{./figs/ls3d_backward.pdf}
%     \label{fig:ls3d-fwd}
%   }
%   \caption{Cumulative Error Distribution (CED) Curves of forward and backward NME for MAFL and LS3D.}
%   \label{fig:ced-curves} \vspace{-0.5em}
% \end{figure*}



% \noindent\textbf{Analysis:} 
% As can be seen in~\Cref{fig:method-quant} our D-ULD++ brings an improvement compared to D-ULD over all pose variations in aggregate. \Cref{fig:method-qual} shows the variations and the learned landmarks are indeed better localized and more accurately matched across poses. 

% % \subsection{Pose-Prediction Proxy Task}
% % Keypoints provide important local information contained in an image. The set of keypoints detected in an image frequently can be used to predict image-level information like pose, emotion expressed etc. 

% % Motivated by this, we propose a proxy task to explore whether the predicted keypoints learned from the network so-far actually are able to predict pose. To this end we use a variational auto-encoder (VAE) to encode and then reconstruct the keypoint heat map predicted by $\Psi_d$. The VAE is trained via a standard ELBO loss~\cite{kingma2013auto}. 

% % Once trained, we show whether the latent codes indeed represent poses by performing a K-Means clustering of the latent codes and checking whether the latent codes within each cluster correspond to similar poses. 

% % \TODO{Maybe add a figure/table here.}



% %\subsection{Pose Pseudo-Label Self-Training} 
% %The keypoints learned from the previous step are used in this step to learn image-level encodings for each image of the dataset. Then, like in the previous step, we alternate between clustering these encodings and using the resulting cluster pseudo-labels to self-train the network. Our underlying motivation behind this step is, to exploit the pose information contained in these keypoints. We show that the clusters in many cases capture similar poses, allowing for an additional pose-based pseudo-label supervision to the network. 

% % \paragraph{VAE based Keypoint Encoding} We first encode the keypoints of each image via a VAE. The input to the VAE is the heatmap of the learned keypoints, which is obtained by splatting Gaussians centered on the keypoints for each image. The VAE learns to predict the keypoint heatmap by minimizing the standard ELBO loss~\cite{}. The latent codes obtained for each image in the process are stored for subsequent clustering. We denote $\mathbf{l}_j$ as the latent code for image $\mathbf{x}_j$.

